Gradient Q$(\sigma, \lambda)$: A Unified Algorithm with Function Approximation for Reinforcement Learning

Full-sampling (e.g., Q-learning) and pure-expectation (e.g., Expected Sarsa) algorithms are efficient and frequently used techniques in reinforcement learning. Q$(\sigma,\lambda)$ is the first approach unifies them with eligibility trace through the sampling degree $\sigma$. However, it is limited to the tabular case, for large-scale learning, the Q$(\sigma,\lambda)$ is too expensive to require a huge volume of tables to accurately storage value functions. To address above problem, we propose a GQ$(\sigma,\lambda)$ that extends tabular Q$(\sigma,\lambda)$ with linear function approximation. We prove the convergence of GQ$(\sigma,\lambda)$. Empirical results on some standard domains show that GQ$(\sigma,\lambda)$ with a combination of full-sampling with pure-expectation reach a better performance than full-sampling and pure-expectation methods.

==> convergence.tex <==
\section{Convergence Analysis}





In this section, we prove the convergence of the proposed Algorithm \ref{alg:algorithm1}.
In order to present the convergent result, we need some additional assumptions.
\begin{assumption}
    \label{ass:positive_lr}
    The positive sequence $\{\alpha_{k}\}_{k\ge0}$, $\{\beta_{k}\}_{k\ge0}$ satisfy $\sum_{k=0}^{\infty}\alpha_{k}=\sum_{k=0}^{\infty}\beta_{k}=\infty,\sum_{k=0}^{\infty}\alpha^{2}_{k}<\infty,\sum_{k=0}^{\infty}\beta^{2}_{k}<\infty$
    with probability one.
\end{assumption}


\begin{assumption}[Boundedness of Feature, Reward and Parameters\cite{liu2015finite}]
    \label{ass:boundedness}
    (1)The features $\{\phi_{t}, \phi_{t+1}\}_{t\ge0}$ have uniformly bounded second moments, where $\phi_{t}=\phi(S_{t}),\phi_{t+1}=\phi(S_{t+1})$.
    (2)The reward function has uniformly bounded second moments.
    (3)There exists bounded $D_{\theta}\times D_{\omega}$,such that $\forall (\theta,\omega)\in D_{\theta}\times D_{\omega}$.
\end{assumption}
Assumption \ref{ass:boundedness} guarantees that the matrices $A_{\sigma}$ and $M$, and vector $b_{\sigma}$ are uniformly bounded.
After some simple algebra, we have $A_{\sigma}=\mathbb{E}[e_{k}\Delta_{k,\sigma}]$, we provide its proof in Appendix C.
The following Assumption \ref{invA} implies $A_{\sigma}^{-1}$ is well-defined.
\begin{assumption}
    \label{invA}
    $A_{\sigma}=\mathbb{E}[e_{k}\Delta_{k,\sigma}]$ is non-singular, where $\Delta_{k,\sigma}$ is defined in Eq.(\ref{Delta}).
\end{assumption}








\begin{theorem}[Convergence of Algorithm \ref{alg:algorithm1}]
    \label{theorem2}
    Consider the iteration $(\theta_{k},\omega_k)$ generated by (\ref{gq_update1}) and (\ref{gq_update2}), if $\beta_{k}=\eta_{k}\alpha_{k}$, $\eta_{k}\rightarrow0$, as $k\rightarrow\infty$ , and $\alpha_{k},\beta_k$ satisfies Assumption \ref{ass:positive_lr}. 
    The sequence $\{(\phi_{k},R_{k},\phi_{k+1})\}_{k\ge0}$ satisfies Assumption \ref{ass:boundedness}.
    Furthermore, $A_{\sigma}=\mathbb{E}[e_{k}\Delta_{k,\sigma}]$ satisfies Assumption \ref{invA}.
        Let $G(\omega,\theta)=A^{T}_{\sigma}M^{-1}A_{\sigma}\theta$,
    $H(\omega,\theta)=A_{\sigma}\theta+b_{\sigma}-M \omega$ 
    Then $(\theta_{k},\omega_k)$ converges to $(\theta^{*},\omega^{*})$ with probability one, 
    where $(\theta^{*},\omega^{*})$ is the unique global asymptotically stable equilibrium w.r.t ordinary differential equation (ODE)
    $\dot\theta(t)=G(\Omega(\theta),\theta)$,$\dot\omega(t)=H(\omega,\theta)$ correspondingly, $\Omega(\theta)$ is a function: $ \theta\mapsto M^{-1}(A_{\sigma}\theta+b_\sigma)$.
\end{theorem}


\begin{proof}
    We use the ordinary differential equation (ODE) method \cite{borkar1997stochastic} or Theorem 2 of Chapter 6 in \cite{borkar2009stochastic} to prove above result. Let $M_{k}=\delta_{k}e_{k}-\gamma v_{\sigma}(\theta_{k})\omega_{k}-M^{-1}(A_{\sigma}\theta_{k}+b_{\sigma})$ and 
    $N_{k}=(\hat{A}_{k}-A_{\sigma})\theta_k+(\hat{b}_{k}-b_{\sigma})-(\hat{M}_{k}-M)\omega_{k}$.
    First, we rewrite the iteration (\ref{gq_update1}) and (\ref{gq_update2}) as follows
    \begin{flalign}
    \label{gq_update1_1}
    \theta_{k+1}&=\theta_{k}+\alpha_{k}(M^{-1}(A_{\sigma}\theta_k+b_{\sigma})+M_k)\\
    \label{gq_update2_1}
    \omega_{k+1}&=\omega_{k}+\beta_{k}(H(\theta_{k},\omega_{k})+N_{k}).
    \end{flalign}
    
    
    Now we apply Theorem 2 in \cite{borkar2009stochastic}(or in \cite{borkar1997stochastic}). Theorem 2 requires the verification of the following conditions:
    (I) Both of the functions $G$ and $H$ are Lipschitz functions.
    It is obvious from Assumption \ref{ass:boundedness}-\ref{invA}.
    (II) Let the $\sigma$-field $\mathcal{F}_{k}=\sigma\{\theta_{t},\omega_{t};t\leq k\}$, then $\mathbb{E}[M_{k}|\mathcal{F}_k]=\mathbb{E}[N_{k}|\mathcal{F}_k]=0$. Furthermore, $\{M_{k}\}_{k\in\mathbb{ N}},\{N_{k}\}_{k\in\mathbb{ N}}$, are square-integrable with
    \begin{flalign}
    \label{MN}
    \mathbb{E}[\|M_{k}\|^{2}|\mathcal{F}_{k}],\mathbb{E}[\|N_{k}\|^{2}|\mathcal{F}_{k}]\leq K(1+\|\theta_{k}\|^{2}+\|\omega_{k}\|^{2}),
    \end{flalign}
    for some constant $K > 0$.
    In fact, it is obvious that $\mathbb{E}[M_{k}|\mathcal{F}_k]=\mathbb{E}[N_{k}|\mathcal{F}_k]=0$.
    By Assumption \ref{ass:boundedness}, Eq.(\ref{A_k}) and Eq.(\ref{b_k}), there exists non-negative 
    constant $K_1,K_2,K_3$ such that $\{\|\hat{A}_{k}\|^{2},\|A_{\sigma}\|^{2}\}\leq K_1$,
    $\{\|\hat{b}_{k}\|^{2},\|b_{\sigma}\|^{2}\}\leq K_2$, $\{\|\hat{M}_{k}\|^{2},\|M\|^{2}\}\leq K_3$ which implies all above terms are bounded.
    Then, 
    \begin{flalign} 
    \nonumber
    &\mathbb{E}[\|N_{k}\|^{2}|\mathcal{F}_{k}]\\
    \nonumber
    =&\mathbb{E}\Big[\|(\hat{A}_{k}-A_{\sigma})\theta_{k}+(\hat{b}_{k}-b_{\sigma})-(\hat{M}_{k}-M)\omega_{k}\|^{2}\Big|\mathcal{F}_{k}\Big]\\
    \label{a}
    \leq&\mathbb{E}\Big[\Big(\|(\hat{A}_{k}-A_{\sigma})\theta_{k}\|+\|\hat{b}_{k}-b_{\sigma}  \|  +  \| (\hat{M}_{k}-M)\omega_{k}\|   \Big)^{2}\Big|\mathcal{F}_{k}\Big]\\
    \label{b}
\leq& {\widetilde{K}_1}^{2}(1+\|\theta_{k}\|^{2}+\|\omega_{k}\|^{2}).
    \end{flalign}
    Eq.(\ref{b}) holds due to Assumption \ref{ass:boundedness}, all the terms in Eq.(\ref{a}) is bounded.
    Thus, for a large positive $\widetilde{K}_1$, we have Eq.(\ref{b}).
Also, by Assumption \ref{ass:boundedness}, $R_{k},\phi_k$ have uniformly bounded second,
then $\mathbb{E}[\|M_{k}\|^{2}|\mathcal{F}_{k}]\leq{\widetilde{K}_2}^{2}(1+\|\theta_{k}\|^{2}+\|\omega_{k}\|^{2})$ for some $\widetilde{K}_2>0$.
Thus, Eq.(\ref{MN}) holds.
(III) For each $\theta\in\mathbb{R}^{p}$, the ODE
    $
    \dot \omega(t) = H(\omega, \theta)
    $
    has a unique global asymptotically stable equilibrium $\Omega(\theta)$ such that:
    $\Omega(\theta):\mathbb{R}^{p}\rightarrow\mathbb{R}^{k}$ is Lipschitz.
In fact, for a fixed $\theta$, by Assumption \ref{invA}, 
$\omega^{*}=M^{-1}(A_{\sigma}\theta+b_{\sigma})$ is the unique globally asymptotically stable equilibrium for ODE
$\dot \omega(t) = A_{\sigma}\theta+b_{\sigma}-M\omega(t).$
Let $\Omega(\theta): \theta\mapsto M^{-1}(A_{\sigma}\theta+b_{\sigma})$,
it is easy to verify $\Omega$ is Lipschitz. 
For a fixed $\theta$, let $H_{\infty}(\omega(t),\theta)$ be a function:
$H_{\infty}(\omega,\theta)=\lim_{r\rightarrow\infty}\dfrac{H_{\infty}(r\omega(t),\theta)}{r}=M\omega({t}).$
Now we consider the ODE
\begin{flalign}
\label{ode:h-infty}
\dot{\omega}(t)=H_{\infty}(\omega,\theta)=M\omega(t).
\end{flalign}
By Assumption \ref{invA} implies that $M$ is a positive definite matrix, thus,
for ODE (\ref{ode:h-infty}), origin is a globally asymptotically stable equilibrium.
Since then, we have verified the conditions of Theorem 2.2 in~\cite{borkar2000ode}, then the following almost surely as $t\rightarrow\infty$,
$
\|\omega_{t}-\omega^{*}\|\rightarrow0,
$
which illustrates the convergence of iteration (\ref{gq_update2}).
(IV)The ODE $\dot \theta(t) =G\big(\Omega(\theta(t)),\theta(t)\big)$ has a unique global asymptotically stable equilibrium $\theta^{*}$.
Now, we consider the iteration (\ref{gq_update1_1})
associated with the following ODE
$
\dot{\theta}(t)=(\gamma\mathbb{E}[\sigma\phi_{k+1}+(1-\sigma)\mathbb{E}_{\pi}[\phi(S_{k+1},\cdot)]]e_{k}^{T}M^{-1}-I)\mathbb{E}[\delta_{k}e_{k}|\theta(t)]
$, which can be rewritten as 
\begin{flalign}
\label{ode-theta-1}
    \dot{\theta}(t)&=\mathbb{E}[\Delta_{k,\sigma}e_{k}^{T}]M^{-1}(A_{\sigma}\theta(t)+b_\sigma)
    \\
    \label{ode-theta-2}
    &=A^{T}_{\sigma}M^{-1}(A_{\sigma}\theta(t)+b_\sigma)
    \overset{\text{def}}=G(\theta(t)),
\end{flalign}
where Eq.(\ref{ode-theta-2}) holds due to $\mathbb{E}[\delta_{k}e_{k}|\theta(t)]=A_{\sigma}\theta(t)+b_\sigma$.
By Assumption \ref{ass:boundedness}, $A_\sigma$ is invertible, then it is obvious $\theta^{*}=-A_{\sigma}^{-1}b_{\sigma}$ is the unique global asymptotically stable equilibrium of ODE (\ref{ode-theta-2}). Let $G_{\infty}(\theta)$ be a function defined by 
$
    G_{\infty}(\theta)=\lim_{r\rightarrow\infty}\frac{G(r\theta,\omega)}{r}
$, thus $G_{\infty}(\theta)=A^{T}_{\sigma} MM^{-1} A_{\sigma}\theta$.
Now we consider the following ODE
\begin{flalign}
    \label{ode-G}
    \dot{\theta}(t)=G_{\infty}(\theta(t)).
\end{flalign}
By Assumption \ref{ass:boundedness}, $A_\sigma$ is invertible and $M^{-1}$ is positive definition, thus $A^{T}_{\sigma} M^{-1} A_{\sigma}$ is also positive definition.
Thus the ODE (\ref{ode-G}) has unique global asymptotically stable equilibrium: origin point.
\end{proof}





==> preliminary.tex <==
\section{Preliminary}
We consider the stochastic multi-bandit (MAB) problem with $K\ge2$ arms.
At each time step $t\in\mathbb{N}$, the agent selects an arm $k\in[K]\overset{\text{def}}=\{1,2,\cdots,K\}$.
Then the agent receives a random real-valued reward $X_{t,k}$ according to an unknown (fixed) distribution $\nu_{k}$ with expectation $\mu_{k}=\mathbb{E}[X_{t,k}]$.
The random rewards are independent identically distributed for each arm is played repeatedly, 
and independent of the plays of the other arms.
We assume that there is an unique optimal arm $k^{*}$ satisfies that $\mu^{*}=\mu_{k^{*}}=\max_{k\in[K]}\mu_{k}$.


\subsection{Unimodal Structure}

In this paper, we mainly focus on the \emph{unimodal} bandit problem where the expected reward function is unimodal over a partially order set of arms, 
which is an important class of problems has been studied by \cite{yu2011unimodal,combes2014unimodal}.
Let $\mathcal{G}=(\mathcal{V},\mathcal{E})$ be an undirected graph, where $\mathcal{V}=[K]$ is the set of vertices correspond to arms, and 
an edge $(i,j)\in\mathcal{E}$ characterizes a partial order between the expected rewards of the arm $i$ and $j$.
Let $\nu=(\nu_{1},\cdots,\nu_{K})$, the partial order of $\mathcal{G}$ is unknown 
since the reward distribution vector $\nu$ is a priori unknown.
The unimodal structure is made precise in the following Assumption \ref{ass-unimodal}.


\begin{assumption}[Unimodality]
\label{ass-unimodal}
Let $\mathcal{G}=(\mathcal{V},\mathcal{E})$ be an undirected graph.
The expected reward function is unimodal along every path $P=(k_1,\cdots,k_m)$ contains $k^{*}$,
such that
\[\mu_{k_1}<\mu_{k_2}<\cdots<\mu_{k^{*}},\mu_{k^{*}}>\cdots>\mu_{k_{j-1}}>\mu_{k_m},\]
where $(k_{i},k_{i+1})\in\mathcal{E},1\leq i\leq m-1$.
\end{assumption}


This unimodality includes the classic unimodality which is a special case when $\mathcal{G}$ is just a line.


\subsection{Regret}

The performance of a policy $\pi$ for MAB problem is measured by its regret.
Let $\mathcal{A}=\{ k_{1},k_{2},\cdots,k_{T}\}$ be the sequence generated by $\pi$, where $k_{i}\in[K],i=1,2,\cdots,T$.
The regret of policy $\pi$ on a bandit is defined as 
\[R_{\pi}(T)=T\mu^{*}-\mathbb{E}[\sum_{i=1}^{T}X_{i,k_i}],\]
where the expectation is taken with respect to the measure on outcomes induced by the interaction of $\pi$ and $\nu$.

We now present the lower bound of $R_{\pi}(T)$ over unimodal bandit problem.
Without loss of generality, we consider the uniformly good policy \cite{lai1985asymptotically}, i.e. $R_{\pi}(T)=o(T^{a})$, for all $a>0$.
We use $N(i)$ to denote the neighborhood of arm $i$, specifically, $N(i)=\{j|(i,j)\in\mathcal{E}\}$.


\begin{theorem}\emph{\cite{combes2014unimodal}}
Let $\pi$ be a uniformly good policy.
For given unimodal bandit $\mathcal{G}=(\mathcal{V},\mathcal{E})$, the following holds,
\begin{flalign}
\label{lower-bound}
\lim_{T\rightarrow\infty}\inf \frac{R_{\pi}(T)}{\log(T)}\ge\sum_{k\in N(k^*)}\frac{\mu^*-\mu_k}{KL(\mu_{k},\mu^*)},
\end{flalign}
where $KL(\mu_{k},\mu^*)=\mu_{k}\log\frac{\mu_k}{\mu^*}+(1-\mu_{k})\log\frac{1-\mu_k}{1-\mu^*}$ is KL-divergence number between Bernoulli distributions of respective means $\mu_k$ and $\mu^*$.
\end{theorem}


==> rw.tex <==
\section{Related Work}
